An Information-theoretic Approach to Distribution Shifts

Safely deploying machine learning models to the real world is often a challenging process. Models trained with data obtained from a specific geographic location tend to fail when queried with data obtained elsewhere, agents trained in a simulation can struggle to adapt when deployed in the real world or novel environments, and neural networks that are fit to a subset of the population might carry some selection bias into their decision process. In this work, we describe the problem of data shift from a novel information-theoretic perspective by (i) identifying and describing the different sources of error, (ii) comparing some of the most promising objectives explored in the recent domain generalization, and fair classification literature. From our theoretical analysis and empirical evaluation, we conclude that the model selection procedure needs to be guided by careful considerations regarding the observed data, the factors used for correction, and the structure of the data-generating process.

==> biblio_all.tex <==
@ARTICLE{Long2017,
       author = {{Long}, Mingsheng and {Cao}, Zhangjie and {Wang}, Jianmin and
         {Jordan}, Michael I.},
        title = "{Conditional Adversarial Domain Adaptation}",
     journal = {arXiv e-prints},
     keywords = {Computer Science - Machine Learning},
         year = 2017
}

@article{Krueger2020,
  author    = {David Krueger and
               Ethan Caballero and
               J{\"{o}}rn{-}Henrik Jacobsen and
               Amy Zhang and
               Jonathan Binas and
               R{\'{e}}mi Le Priol and
               Aaron C. Courville},
  title     = {Out-of-Distribution Generalization via Risk Extrapolation (REx)},
  journal   = {CoRR},
  volume    = {abs/2003.00688},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.00688},
  archivePrefix = {arXiv},
  eprint    = {2003.00688},
  timestamp = {Tue, 01 Sep 2020 23:31:48 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2003-00688.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Li2018,
  author    = {Haoliang Li and
               Sinno Jialin Pan and
               Shiqi Wang and
               Alex C. Kot},
  title     = {Domain Generalization With Adversarial Feature Learning},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {5400--5409},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Li\_Domain\_Generalization\_With\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00566},
  timestamp = {Sat, 05 Sep 2020 18:03:36 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/LiPWK18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Peters2015,
  title={Causal inference by using invariant prediction: identification and confidence intervals},
  author={Peters, Jonas and B{\"u}hlmann, Peter and Meinshausen, Nicolai},
  journal={Journal of the Royal Statistical Society. Series B (Statistical Methodology)},
  pages={947--1012},
  year={2016},
  publisher={JSTOR}
}

@article{Tishby2015,
  author    = {Naftali Tishby and
               Noga Zaslavsky},
  title     = {Deep Learning and the Information Bottleneck Principle},
  journal   = {CoRR},
  volume    = {abs/1503.02406},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.02406},
  archivePrefix = {arXiv},
  eprint    = {1503.02406},
  timestamp = {Mon, 13 Aug 2018 16:48:20 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/TishbyZ15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Alemi2016,
  author    = {Alexander A. Alemi and
               Ian Fischer and
               Joshua V. Dillon and
               Kevin Murphy},
  title     = {Deep Variational Information Bottleneck},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/forum?id=HyxQzBceg},
  timestamp = {Thu, 25 Jul 2019 14:25:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/AlemiFD017.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Du2020,
  author    = {Ying{-}Jun Du and
               Jun Xu and
               Huan Xiong and
               Qiang Qiu and
               Xiantong Zhen and
               Cees G. M. Snoek and
               Ling Shao},
  editor    = {Andrea Vedaldi and
               Horst Bischof and
               Thomas Brox and
               Jan{-}Michael Frahm},
  title     = {Learning to Learn with Variational Information Bottleneck for Domain
               Generalization},
  booktitle = {Computer Vision - {ECCV} 2020 - 16th European Conference, Glasgow,
               UK, August 23-28, 2020, Proceedings, Part {X}},
  series    = {Lecture Notes in Computer Science},
  volume    = {12355},
  pages     = {200--216},
  publisher = {Springer},
  year      = {2020},
  url       = {https://doi.org/10.1007/978-3-030-58607-2\_12},
  doi       = {10.1007/978-3-030-58607-2\_12},
  timestamp = {Wed, 03 Feb 2021 15:08:01 +0100},
  biburl    = {https://dblp.org/rec/conf/eccv/DuXXQZS020.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Song2019,
  author    = {Yuxuan Song and
               Lantao Yu and
               Zhangjie Cao and
               Zhiming Zhou and
               Jian Shen and
               Shuo Shao and
               Weinan Zhang and
               Yong Yu},
  editor    = {Giuseppe De Giacomo and
               Alejandro Catal{\'{a}} and
               Bistra Dilkina and
               Michela Milano and
               Sen{\'{e}}n Barro and
               Alberto Bugar{\'{\i}}n and
               J{\'{e}}r{\^{o}}me Lang},
  title     = {Improving Unsupervised Domain Adaptation with Variational Information
               Bottleneck},
  booktitle = {{ECAI} 2020 - 24th European Conference on Artificial Intelligence,
               29 August-8 September 2020, Santiago de Compostela, Spain, August
               29 - September 8, 2020 - Including 10th Conference on Prestigious
               Applications of Artificial Intelligence {(PAIS} 2020)},
  series    = {Frontiers in Artificial Intelligence and Applications},
  volume    = {325},
  pages     = {1499--1506},
  publisher = {{IOS} Press},
  year      = {2020},
  url       = {https://doi.org/10.3233/FAIA200257},
  doi       = {10.3233/FAIA200257},
  timestamp = {Fri, 29 Jan 2021 22:09:11 +0100},
  biburl    = {https://dblp.org/rec/conf/ecai/SongYCZSS0020.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Buhlmann2018,
  title={Invariance, causality and robustness},
  author={B{\"u}hlmann, Peter and others},
  journal={Statistical Science},
  volume={35},
  number={3},
  pages={404--426},
  year={2020},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{Magliacane2017,
  author    = {Sara Magliacane and
               Thijs van Ommen and
               Tom Claassen and
               Stephan Bongers and
               Philip Versteeg and
               Joris M. Mooij},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Domain Adaptation by Using Causal Inference to Predict Invariant Conditional
               Distributions},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {10869--10879},
  year      = {2018},
  url       = {https://proceedings.neurips.cc/paper/2018/hash/39e98420b5e98bfbdc8a619bef7b8f61-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/MagliacaneOCBVM18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Arjovsky2019,
  author    = {Mart{\'{\i}}n Arjovsky and
               L{\'{e}}on Bottou and
               Ishaan Gulrajani and
               David Lopez{-}Paz},
  title     = {Invariant Risk Minimization},
  journal   = {CoRR},
  volume    = {abs/1907.02893},
  year      = {2019},
  url       = {http://arxiv.org/abs/1907.02893},
  archivePrefix = {arXiv},
  eprint    = {1907.02893},
  timestamp = {Mon, 08 Jul 2019 14:12:33 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1907-02893.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Rosenfeld2020,
  author    = {Elan Rosenfeld and
               Pradeep Ravikumar and
               Andrej Risteski},
  title     = {The Risks of Invariant Risk Minimization},
  journal   = {CoRR},
  volume    = {abs/2010.05761},
  year      = {2020},
  url       = {https://arxiv.org/abs/2010.05761},
  archivePrefix = {arXiv},
  eprint    = {2010.05761},
  timestamp = {Tue, 20 Oct 2020 15:08:10 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2010-05761.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Zhao2019,
  author    = {Han Zhao and
               Remi Tachet des Combes and
               Kun Zhang and
               Geoffrey J. Gordon},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {On Learning Invariant Representations for Domain Adaptation},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {7523--7532},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/zhao19a.html},
  timestamp = {Sun, 23 Jun 2019 08:14:09 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/0002CZG19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Johansson2019,
  author    = {Fredrik D. Johansson and
               David A. Sontag and
               Rajesh Ranganath},
  editor    = {Kamalika Chaudhuri and
               Masashi Sugiyama},
  title     = {Support and Invertibility in Domain-Invariant Representations},
  booktitle = {The 22nd International Conference on Artificial Intelligence and Statistics,
               {AISTATS} 2019, 16-18 April 2019, Naha, Okinawa, Japan},
  series    = {Proceedings of Machine Learning Research},
  volume    = {89},
  pages     = {527--536},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v89/johansson19a.html},
  timestamp = {Fri, 15 Nov 2019 17:16:05 +0100},
  biburl    = {https://dblp.org/rec/conf/aistats/JohanssonSR19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Azizzadenesheli2019,
  author    = {Kamyar Azizzadenesheli and
               Anqi Liu and
               Fanny Yang and
               Animashree Anandkumar},
  title     = {Regularized Learning for Domain Adaptation under Label Shifts},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/forum?id=rJl0r3R9KX},
  timestamp = {Thu, 25 Jul 2019 14:25:47 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/Azizzadenesheli19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Gulrajani2020,
  author    = {Ishaan Gulrajani and
               David Lopez{-}Paz},
  title     = {In Search of Lost Domain Generalization},
  journal   = {CoRR},
  volume    = {abs/2007.01434},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.01434},
  archivePrefix = {arXiv},
  eprint    = {2007.01434},
  timestamp = {Mon, 06 Jul 2020 15:26:01 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-01434.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Koyama2020,
  author    = {Masanori Koyama and
               Shoichiro Yamaguchi},
  title     = {Out-of-Distribution Generalization with Maximal Invariant Predictor},
  journal   = {CoRR},
  volume    = {abs/2008.01883},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.01883},
  archivePrefix = {arXiv},
  eprint    = {2008.01883},
  timestamp = {Fri, 07 Aug 2020 15:07:21 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2008-01883.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{YLi2018,
  author    = {Ya Li and
               Xinmei Tian and
               Mingming Gong and
               Yajing Liu and
               Tongliang Liu and
               Kun Zhang and
               Dacheng Tao},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Deep Domain Generalization via Conditional Invariant Adversarial Networks},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XV}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11219},
  pages     = {647--663},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01267-0\_38},
  doi       = {10.1007/978-3-030-01267-0\_38},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/LiTGLLZT18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Mehrabi2019,
  author    = {Ninareh Mehrabi and
               Fred Morstatter and
               Nripsuta Saxena and
               Kristina Lerman and
               Aram Galstyan},
  title     = {A Survey on Bias and Fairness in Machine Learning},
  journal   = {CoRR},
  volume    = {abs/1908.09635},
  year      = {2019},
  url       = {http://arxiv.org/abs/1908.09635},
  archivePrefix = {arXiv},
  eprint    = {1908.09635},
  timestamp = {Thu, 29 Aug 2019 16:32:34 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1908-09635.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Koh2020,
  author    = {Pang Wei Koh and
               Shiori Sagawa and
               Henrik Marklund and
               Sang Michael Xie and
               Marvin Zhang and
               Akshay Balsubramani and
               Weihua Hu and
               Michihiro Yasunaga and
               Richard Lanas Phillips and
               Sara Beery and
               Jure Leskovec and
               Anshul Kundaje and
               Emma Pierson and
               Sergey Levine and
               Chelsea Finn and
               Percy Liang},
  title     = {{WILDS:} {A} Benchmark of in-the-Wild Distribution Shifts},
  journal   = {CoRR},
  volume    = {abs/2012.07421},
  year      = {2020},
  url       = {https://arxiv.org/abs/2012.07421},
  archivePrefix = {arXiv},
  eprint    = {2012.07421},
  timestamp = {Sat, 02 Jan 2021 15:43:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2012-07421.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Bengio2019,
  author    = {Yoshua Bengio and
               Tristan Deleu and
               Nasim Rahaman and
               Nan Rosemary Ke and
               S{\'{e}}bastien Lachapelle and
               Olexa Bilaniuk and
               Anirudh Goyal and
               Christopher J. Pal},
  title     = {A Meta-Transfer Objective for Learning to Disentangle Causal Mechanisms},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  publisher = {OpenReview.net},
  year      = {2020},
  url       = {https://openreview.net/forum?id=ryxWIgBFPS},
  timestamp = {Thu, 07 May 2020 17:11:48 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/BengioDRKLBGP20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Hardt2016,
  author    = {Moritz Hardt and
               Eric Price and
               Nati Srebro},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Equality of Opportunity in Supervised Learning},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {3315--3323},
  year      = {2016},
  url       = {https://proceedings.neurips.cc/paper/2016/hash/9d2682367c3935defcb1f9e247a97c0d-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:22 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/HardtPNS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Woodworth2017,
  author    = {Blake E. Woodworth and
               Suriya Gunasekar and
               Mesrob I. Ohannessian and
               Nathan Srebro},
  editor    = {Satyen Kale and
               Ohad Shamir},
  title     = {Learning Non-Discriminatory Predictors},
  booktitle = {Proceedings of the 30th Conference on Learning Theory, {COLT} 2017,
               Amsterdam, The Netherlands, 7-10 July 2017},
  series    = {Proceedings of Machine Learning Research},
  volume    = {65},
  pages     = {1920--1953},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v65/woodworth17a.html},
  timestamp = {Wed, 29 May 2019 08:41:46 +0200},
  biburl    = {https://dblp.org/rec/conf/colt/WoodworthGOS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Kilbertus2017,
  author    = {Niki Kilbertus and
               Mateo Rojas{-}Carulla and
               Giambattista Parascandolo and
               Moritz Hardt and
               Dominik Janzing and
               Bernhard Sch{\"{o}}lkopf},
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {Avoiding Discrimination through Causal Reasoning},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, December 4-9, 2017,
               Long Beach, CA, {USA}},
  pages     = {656--666},
  year      = {2017},
  url       = {https://proceedings.neurips.cc/paper/2017/hash/f5f8590cd58a54e94377e6ae2eded4d9-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/KilbertusRPHJS17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{Quionero2009,
author = {Quionero-Candela, Joaquin and Sugiyama, Masashi and Schwaighofer, Anton and Lawrence, Neil D.},
title = {Dataset Shift in Machine Learning},
year = {2009},
isbn = {0262170051},
publisher = {The MIT Press}
}

@article{Widmer1996,
  author    = {Gerhard Widmer and
               Miroslav Kubat},
  title     = {Learning in the Presence of Concept Drift and Hidden Contexts},
  journal   = {Mach. Learn.},
  volume    = {23},
  number    = {1},
  pages     = {69--101},
  year      = {1996},
  url       = {https://doi.org/10.1007/BF00116900},
  doi       = {10.1007/BF00116900},
  timestamp = {Mon, 02 Mar 2020 16:30:07 +0100},
  biburl    = {https://dblp.org/rec/journals/ml/WidmerK96.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Moreno2012,
  author    = {Jose G. Moreno{-}Torres and
               Troy Raeder and
               Roc{\'{\i}}o Ala{\'{\i}}z{-}Rodr{\'{\i}}guez and
               Nitesh V. Chawla and
               Francisco Herrera},
  title     = {A unifying view on dataset shift in classification},
  journal   = {Pattern Recognit.},
  volume    = {45},
  number    = {1},
  pages     = {521--530},
  year      = {2012},
  url       = {https://doi.org/10.1016/j.patcog.2011.06.019},
  doi       = {10.1016/j.patcog.2011.06.019},
  timestamp = {Mon, 24 Feb 2020 08:28:46 +0100},
  biburl    = {https://dblp.org/rec/journals/pr/Moreno-TorresRACH12.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Shimodaira2000,
title = "Improving predictive inference under covariate shift by weighting the log-likelihood function",
journal = "Journal of Statistical Planning and Inference",
year = "2000",
issn = "0378-3758",
doi = "https://doi.org/10.1016/S0378-3758(00)00115-4",
author = "Hidetoshi Shimodaira",
}

@article{Ganin2015,
  author    = {Yaroslav Ganin and
               Evgeniya Ustinova and
               Hana Ajakan and
               Pascal Germain and
               Hugo Larochelle and
               Fran{\c{c}}ois Laviolette and
               Mario Marchand and
               Victor S. Lempitsky},
  title     = {Domain-Adversarial Training of Neural Networks},
  journal   = {J. Mach. Learn. Res.},
  volume    = {17},
  pages     = {59:1--59:35},
  year      = {2016},
  url       = {http://jmlr.org/papers/v17/15-239.html},
  timestamp = {Wed, 10 Jul 2019 15:28:07 +0200},
  biburl    = {https://dblp.org/rec/journals/jmlr/GaninUAGLLML16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Louizos2015,
  author    = {Christos Louizos and
               Kevin Swersky and
               Yujia Li and
               Max Welling and
               Richard S. Zemel},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {The Variational Fair Autoencoder},
  booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
               San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
  year      = {2016},
  url       = {http://arxiv.org/abs/1511.00830},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LouizosSLWZ15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Moyer2018,
  author    = {Daniel Moyer and
               Shuyang Gao and
               Rob Brekelmans and
               Aram Galstyan and
               Greg Ver Steeg},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {Invariant Representations without Adversarial Training},
  booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {9102--9111},
  year      = {2018},
  url       = {https://proceedings.neurips.cc/paper/2018/hash/415185ea244ea2b2bedeb0449b926802-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/MoyerGBGS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Lum2016,
  author    = {Kristian Lum and
               James E. Johndrow},
  title     = {A statistical framework for fair predictive algorithms},
  journal   = {CoRR},
  volume    = {abs/1610.08077},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.08077},
  archivePrefix = {arXiv},
  eprint    = {1610.08077},
  timestamp = {Mon, 13 Aug 2018 16:46:00 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LumJ16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Verma2018,
  author    = {Sahil Verma and
               Julia Rubin},
  editor    = {Yuriy Brun and
               Brittany Johnson and
               Alexandra Meliou},
  title     = {Fairness definitions explained},
  booktitle = {Proceedings of the International Workshop on Software Fairness, FairWare@ICSE
               2018, Gothenburg, Sweden, May 29, 2018},
  pages     = {1--7},
  publisher = {{ACM}},
  year      = {2018},
  url       = {https://doi.org/10.1145/3194770.3194776},
  doi       = {10.1145/3194770.3194776},
  timestamp = {Sun, 25 Oct 2020 22:57:40 +0100},
  biburl    = {https://dblp.org/rec/conf/icse/VermaR18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Kingma2013,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6114},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaW13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@book{Barocas2018,
  title = {Fairness and Machine Learning},
  author = {Solon Barocas and Moritz Hardt and Arvind Narayanan},
  publisher = {fairmlbook.org},
  note = {\url{http://www.fairmlbook.org}},
  year = {2018}
}

@article{Dwork2011,
  author    = {Cynthia Dwork and
               Moritz Hardt and
               Toniann Pitassi and
               Omer Reingold and
               Richard S. Zemel},
  title     = {Fairness Through Awareness},
  journal   = {CoRR},
  volume    = {abs/1104.3913},
  year      = {2011},
  url       = {http://arxiv.org/abs/1104.3913},
  archivePrefix = {arXiv},
  eprint    = {1104.3913},
  timestamp = {Mon, 13 Aug 2018 16:48:46 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1104-3913.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Dwork2006,
author="Dwork, Cynthia",
editor="Bugliesi, Michele
and Preneel, Bart
and Sassone, Vladimiro
and Wegener, Ingo",
title="Differential Privacy",
booktitle="Automata, Languages and Programming",
year="2006",
publisher="Springer Berlin Heidelberg",
pages="1-12",
isbn="978-3-540-35908-1"
}

@inproceedings{Corbett2017,
  author    = {Sam Corbett{-}Davies and
               Emma Pierson and
               Avi Feller and
               Sharad Goel and
               Aziz Huq},
  title     = {Algorithmic Decision Making and the Cost of Fairness},
  booktitle = {Proceedings of the 23rd {ACM} {SIGKDD} International Conference on
               Knowledge Discovery and Data Mining, Halifax, NS, Canada, August 13
               - 17, 2017},
  pages     = {797--806},
  publisher = {{ACM}},
  year      = {2017},
  url       = {https://doi.org/10.1145/3097983.3098095},
  doi       = {10.1145/3097983.3098095},
  timestamp = {Fri, 25 Dec 2020 01:14:16 +0100},
  biburl    = {https://dblp.org/rec/conf/kdd/Corbett-DaviesP17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{Huszar2019,
 author = {Huszár, Ferenc},
 year = {2019},
 title = {Invariant Risk Minimization: An Information Theoretic View},
 url = {https://www.inference.vc/invariant-risk-minimization/}
}

@article{Chouldechova2016,
  author    = {Alexandra Chouldechova},
  title     = {Fair Prediction with Disparate Impact: {A} Study of Bias in Recidivism
               Prediction Instruments},
  journal   = {Big Data},
  volume    = {5},
  number    = {2},
  pages     = {153--163},
  year      = {2017},
  url       = {https://doi.org/10.1089/big.2016.0047},
  doi       = {10.1089/big.2016.0047},
  timestamp = {Thu, 28 Nov 2019 10:42:39 +0100},
  biburl    = {https://dblp.org/rec/journals/bigdata/Chouldechova17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Muandet2013,
  author    = {Krikamol Muandet and
               David Balduzzi and
               Bernhard Sch{\"{o}}lkopf},
  title     = {Domain Generalization via Invariant Feature Representation},
  booktitle = {Proceedings of the 30th International Conference on Machine Learning,
               {ICML} 2013, Atlanta, GA, USA, 16-21 June 2013},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {28},
  pages     = {10--18},
  publisher = {JMLR.org},
  year      = {2013},
  url       = {http://proceedings.mlr.press/v28/muandet13.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/MuandetBS13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Xie2017,
  author    = {Qizhe Xie and
               Zihang Dai and
               Yulun Du and
               Eduard H. Hovy and
               Graham Neubig},
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {Controllable Invariance through Adversarial Feature Learning},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, December 4-9, 2017,
               Long Beach, CA, {USA}},
  pages     = {585--596},
  year      = {2017},
  url       = {https://proceedings.neurips.cc/paper/2017/hash/8cb22bdd0b7ba1ab13d742e22eed8da2-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/XieDDHN17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Ilse2019,
  author    = {Maximilian Ilse and
               Jakub M. Tomczak and
               Christos Louizos and
               Max Welling},
  editor    = {Tal Arbel and
               Ismail Ben Ayed and
               Marleen de Bruijne and
               Maxime Descoteaux and
               Herv{\'{e}} Lombaert and
               Christopher Pal},
  title     = {{DIVA:} Domain Invariant Variational Autoencoders},
  booktitle = {International Conference on Medical Imaging with Deep Learning, {MIDL}
               2020, 6-8 July 2020, Montr{\'{e}}al, QC, Canada},
  series    = {Proceedings of Machine Learning Research},
  volume    = {121},
  pages     = {322--348},
  publisher = {{PMLR}},
  year      = {2020},
  url       = {http://proceedings.mlr.press/v121/ilse20a.html},
  timestamp = {Fri, 27 Nov 2020 16:13:27 +0100},
  biburl    = {https://dblp.org/rec/conf/midl/IlseTLW20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Parascandolo2020,
  author    = {Giambattista Parascandolo and
               Alexander Neitz and
               Antonio Orvieto and
               Luigi Gresele and
               Bernhard Sch{\"{o}}lkopf},
  title     = {Learning explanations that are hard to vary},
  journal   = {CoRR},
  volume    = {abs/2009.00329},
  year      = {2020},
  url       = {https://arxiv.org/abs/2009.00329},
  archivePrefix = {arXiv},
  eprint    = {2009.00329},
  timestamp = {Wed, 16 Sep 2020 15:27:56 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2009-00329.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Darlington1971,
 ISSN = {00220655, 17453984},
 author = {Richard B. Darlington},
 journal = {Journal of Educational Measurement},
 pages = {71-82},
 publisher = {[National Council on Measurement in Education, Wiley]},
 title = {Another Look at "Cultural Fairness"},
 volume = {8},
 year = {1971}
}

@article{Xie2020,
  author    = {Chuanlong Xie and
               Fei Chen and
               Yue Liu and
               Zhenguo Li},
  title     = {Risk Variance Penalization: From Distributional Robustness to Causality},
  journal   = {CoRR},
  volume    = {abs/2006.07544},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.07544},
  archivePrefix = {arXiv},
  eprint    = {2006.07544},
  timestamp = {Wed, 17 Jun 2020 14:28:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-07544.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Wang2018,
  author    = {Mei Wang and
               Weihong Deng},
  title     = {Deep visual domain adaptation: {A} survey},
  journal   = {Neurocomputing},
  volume    = {312},
  pages     = {135--153},
  year      = {2018},
  url       = {https://doi.org/10.1016/j.neucom.2018.05.083},
  doi       = {10.1016/j.neucom.2018.05.083},
  timestamp = {Sat, 11 Aug 2018 00:57:24 +0200},
  biburl    = {https://dblp.org/rec/journals/ijon/WangD18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Santurkar2020,
  author    = {Shibani Santurkar and
               Dimitris Tsipras and
               Aleksander Madry},
  title     = {{BREEDS:} Benchmarks for Subpopulation Shift},
  journal   = {CoRR},
  volume    = {abs/2008.04859},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.04859},
  archivePrefix = {arXiv},
  eprint    = {2008.04859},
  timestamp = {Sun, 16 Aug 2020 17:19:29 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2008-04859.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article {Jean2016,
	author = {Jean, Neal and Burke, Marshall and Xie, Michael and Davis, W. Matthew and Lobell, David B. and Ermon, Stefano},
	title = {Combining satellite imagery and machine learning to predict poverty},
	volume = {353},
	pages = {790-794},
	year = {2016},
	doi = {10.1126/science.aaf7894},
	publisher = {American Association for the Advancement of Science},
	journal = {Science}
}

@inproceedings{Christie2017,
  author    = {Gordon Christie and
               Neil Fendley and
               James Wilson and
               Ryan Mukherjee},
  title     = {Functional Map of the World},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {6172--6180},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Christie\_Functional\_Map\_of\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00646},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/ChristieFWM18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Zech2018,
    author = {Zech, John R. AND Badgeley, Marcus A. AND Liu, Manway AND Costa, Anthony B. AND Titano, Joseph J. AND Oermann, Eric Karl},
    journal = {PLOS Medicine},
    publisher = {Public Library of Science},
    title = {Variable generalization performance of a deep learning model to detect pneumonia in chest radiographs: A cross-sectional study},
    year = {2018}
}

@inproceedings{Perona2018,
  author    = {Sara Beery and
               Grant Van Horn and
               Pietro Perona},
  editor    = {Vittorio Ferrari and
               Martial Hebert and
               Cristian Sminchisescu and
               Yair Weiss},
  title     = {Recognition in Terra Incognita},
  booktitle = {Computer Vision - {ECCV} 2018 - 15th European Conference, Munich,
               Germany, September 8-14, 2018, Proceedings, Part {XVI}},
  series    = {Lecture Notes in Computer Science},
  volume    = {11220},
  pages     = {472--489},
  publisher = {Springer},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-01270-0\_28},
  doi       = {10.1007/978-3-030-01270-0\_28},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/BeeryHP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Buolamwini2018,
  author    = {Joy Buolamwini and
               Timnit Gebru},
  editor    = {Sorelle A. Friedler and
               Christo Wilson},
  title     = {Gender Shades: Intersectional Accuracy Disparities in Commercial Gender
               Classification},
  booktitle = {Conference on Fairness, Accountability and Transparency, {FAT} 2018,
               23-24 February 2018, New York, NY, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {81},
  pages     = {77--91},
  publisher = {{PMLR}},
  year      = {2018},
  url       = {http://proceedings.mlr.press/v81/buolamwini18a.html},
  timestamp = {Wed, 03 Apr 2019 18:17:20 +0200},
  biburl    = {https://dblp.org/rec/conf/fat/BuolamwiniG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Koenecke2020,
  author    = {Allison Koenecke and
               Andrew Nam and
               Emily Lake and
               Joe Nudell and
               Minnie Quartey and
               Zion Mengesha and
               Connor Toups and
               John R. Rickford and
               Dan Jurafsky and
               Sharad Goel},
  title     = {Racial disparities in automated speech recognition},
  journal   = {Proc. Natl. Acad. Sci. {USA}},
  volume    = {117},
  number    = {14},
  pages     = {7684--7689},
  year      = {2020},
  url       = {https://doi.org/10.1073/pnas.1915768117},
  doi       = {10.1073/pnas.1915768117},
  timestamp = {Fri, 25 Dec 2020 01:11:49 +0100},
  biburl    = {https://dblp.org/rec/journals/pnas/KoeneckeNLNQMTR20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Bolukbasi2016,
  author    = {Tolga Bolukbasi and
               Kai{-}Wei Chang and
               James Y. Zou and
               Venkatesh Saligrama and
               Adam Tauman Kalai},
  editor    = {Daniel D. Lee and
               Masashi Sugiyama and
               Ulrike von Luxburg and
               Isabelle Guyon and
               Roman Garnett},
  title     = {Man is to Computer Programmer as Woman is to Homemaker? Debiasing
               Word Embeddings},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {4349--4357},
  year      = {2016},
  url       = {https://proceedings.neurips.cc/paper/2016/hash/a486cd07e4ac3d270571622f4f316ec5-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:22 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/BolukbasiCZSK16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Beede2020,
  author    = {Emma Beede and
               Elizabeth Baylor and
               Fred Hersch and
               Anna Iurchenko and
               Lauren Wilcox and
               Paisan Ruamviboonsuk and
               Laura M. Vardoulakis},
  editor    = {Regina Bernhaupt and
               Florian 'Floyd' Mueller and
               David Verweij and
               Josh Andres and
               Joanna McGrenere and
               Andy Cockburn and
               Ignacio Avellino and
               Alix Goguey and
               Pernille Bj{\o}n and
               Shengdong Zhao and
               Briane Paul Samson and
               Rafal Kocielnik},
  title     = {A Human-Centered Evaluation of a Deep Learning System Deployed in
               Clinics for the Detection of Diabetic Retinopathy},
  booktitle = {{CHI} '20: {CHI} Conference on Human Factors in Computing Systems,
               Honolulu, HI, USA, April 25-30, 2020},
  pages     = {1--12},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3313831.3376718},
  doi       = {10.1145/3313831.3376718},
  timestamp = {Tue, 12 May 2020 12:58:02 +0200},
  biburl    = {https://dblp.org/rec/conf/chi/BeedeBHIWRV20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Popejoy2016,
  title={Genomics is failing on diversity},
  author={A. Popejoy and S. Fullerton},
  journal={Nature},
  year={2016},
  volume={538},
  pages={161-164}
}

@article{Zhang2017,
  author    = {Jing Zhang and
               Victor S. Sheng and
               Qianmu Li and
               Jian Wu and
               Xindong Wu},
  title     = {Consensus algorithms for biased labeling in crowdsourcing},
  journal   = {Inf. Sci.},
  volume    = {382-383},
  pages     = {254--273},
  year      = {2017},
  url       = {https://doi.org/10.1016/j.ins.2016.12.026},
  doi       = {10.1016/j.ins.2016.12.026},
  timestamp = {Sat, 19 Oct 2019 19:19:12 +0200},
  biburl    = {https://dblp.org/rec/journals/isci/ZhangSLWW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Xia2020,
  author    = {Mengzhou Xia and
               Anjalie Field and
               Yulia Tsvetkov},
  editor    = {Lun{-}Wei Ku and
               Cheng{-}Te Li},
  title     = {Demoting Racial Bias in Hate Speech Detection},
  booktitle = {Proceedings of the Eighth International Workshop on Natural Language
               Processing for Social Media, SocialNLP@ACL 2020, Online, July 10,
               2020},
  pages     = {7--14},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://doi.org/10.18653/v1/2020.socialnlp-1.2},
  doi       = {10.18653/v1/2020.socialnlp-1.2},
  timestamp = {Fri, 04 Dec 2020 16:52:28 +0100},
  biburl    = {https://dblp.org/rec/conf/acl-socialnlp/XiaFT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Mahajan2020,
  author    = {Divyat Mahajan and
               Shruti Tople and
               Amit Sharma},
  title     = {Domain Generalization using Causal Matching},
  journal   = {CoRR},
  volume    = {abs/2006.07500},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.07500},
  archivePrefix = {arXiv},
  eprint    = {2006.07500},
  timestamp = {Wed, 17 Jun 2020 14:28:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-07500.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Bloem2019,
  author    = {Benjamin Bloem{-}Reddy and
               Yee Whye Teh},
  title     = {Probabilistic Symmetries and Invariant Neural Networks},
  journal   = {J. Mach. Learn. Res.},
  volume    = {21},
  pages     = {90:1--90:61},
  year      = {2020},
  url       = {http://jmlr.org/papers/v21/19-322.html},
  timestamp = {Wed, 18 Nov 2020 15:58:12 +0100},
  biburl    = {https://dblp.org/rec/journals/jmlr/Bloem-ReddyT20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Cohen2016,
  author    = {Taco Cohen and
               Max Welling},
  editor    = {Maria{-}Florina Balcan and
               Kilian Q. Weinberger},
  title     = {Group Equivariant Convolutional Networks},
  booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
               {ICML} 2016, New York City, NY, USA, June 19-24, 2016},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {48},
  pages     = {2990--2999},
  publisher = {JMLR.org},
  year      = {2016},
  url       = {http://proceedings.mlr.press/v48/cohenc16.html},
  timestamp = {Wed, 29 May 2019 08:41:46 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/CohenW16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Gouk2018,
  author    = {Henry Gouk and
               Eibe Frank and
               Bernhard Pfahringer and
               Michael J. Cree},
  title     = {Regularisation of Neural Networks by Enforcing Lipschitz Continuity},
  journal   = {CoRR},
  volume    = {abs/1804.04368},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.04368},
  archivePrefix = {arXiv},
  eprint    = {1804.04368},
  timestamp = {Mon, 13 Aug 2018 16:47:24 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-04368.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

==> sections/neurips/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The claims point directly to the part of the papers in which they are supported} 
  \item Did you describe the limitations of your work?
    \answerYes{Discussion regarding the assumptions is reported in appendix~\ref{app:pred_info} and in the conclusions.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The whole paper aims to better understand and address the problems of distribution shift and selection bias, which can have negative social impact}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Precise statements are reported in appendix~\ref{app:proofs}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Proofs are reported in appendix~\ref{app:proofs}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code used to compute the results is either publicly available or included in the anonymized URL that is reported in the appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See appendix~\ref{app:nn_train}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Error bars are reported for neural network experiments. The standard deviation for the results obtained with direct optimization is negligible.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See appendix~\ref{app:nn_train}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{The Code License is included in the repository.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The procedure used to produce the different versions of the CMNIST dataset is accessible from the released code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{The MNIST dataset is publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

